Towards Off-Policy Reinforcement Learning for Ranking Policies with Human Feedback

Probabilistic learning to rank (LTR) has been the dominating approach for optimizing the ranking metric, but cannot maximize long-term rewards. Reinforcement learning models have been proposed to maximize user long-term rewards by formulating the recommendation as a sequential decision-making problem, but could only achieve inferior accuracy compared to LTR counterparts, primarily due to the lack of online interactions and the characteristics of ranking. In this paper, we propose a new off-policy value ranking (VR) algorithm that can simultaneously maximize user long-term rewards and optimize the ranking metric offline for improved sample efficiency in a unified Expectation-Maximization (EM) framework. We theoretically and empirically show that the EM process guides the leaned policy to enjoy the benefit of integration of the future reward and ranking metric, and learn without any online interactions. Extensive offline and online experiments demonstrate the effectiveness of our methods.

==> Related_Work.tex <==
%!TEX root = ./OffIine_Ranking.tex
% \section{Related Work}
% \label{sec:RW}

% \subsection{RL for Recommendation}
% There are two major families of model-free reinforcement learning approaches, i.e., value-based and policy-based. Value-based approaches such as Q-learning~\cite{mnih2013playing},  deterministic policy gradient~\cite{lillicrap2015continuous} and soft actor-critic~\cite{haarnoja2018soft}, typically use a Q function approximator to learn the state-action value function. These methods fail on offline datasets due to overestimation issue~\cite{fu2020d4rl}.  The policy-based methods such as policy gradient~\cite{williams1992simple},  parameterize the policy directly and learn the policy to maximize expected long-term reward. When it comes to the recommendation, Some attempts propose to model recommendation task via  Q-learning~\cite{DBLP:conf/kdd/ZhaoZDXTY18,DBLP:conf/sigir/ZhouDC0RTH020} and deep deterministic policy gradient~\cite{zhao2018ac}. \citeauthor{DBLP:conf/wsdm/ChenBCJBC19} proposes to utilize the off-policy policy gradient~\cite{DBLP:conf/wsdm/ChenBCJBC19} to correct the system biases
% in the logged  feedback and maximize expected long-term reward. However, as mentioned by~\cite{DBLP:conf/wsdm/ChenBCJBC19,jeunen2020joint}, the actions with zero-reward will not contribute to the gradient update. Thus, it is not suitable for ranking. Recently, some works~\cite{DBLP:conf/nips/BaiGW19,DBLP:conf/icml/Chen0LJQS19,DBLP:conf/wsdm/ZouXDZB0NY20} also try to solve the  recommendation task via model-based RL algorithms. However, it is difficult to simulate the user environment  and these methods heavily depend on the accuracy of the estimate of the environment. By contrast, in this paper, our  algorithm are model-free RL algorithms   and can directly optimize the ranking metric offline without online interactions. 

% \subsection{Batch Bandits and Reinforcement Learning}
% Our work is  related to the batch bandit, which can be  viewed as a special case of RL with single-step environments.   \citep{DBLP:journals/jmlr/SwaminathanJ15} proposes counterfactual risk minimization (CRM), which can directly learn unbiased policy from logged feedback without interactions. Various methods~\cite{dudik2011doubly,swaminathan2015self,joachims2018deep} have been proposed to address the problem of batch bandits and achieve better bias-variance trade-off.  \citeauthor{jeunen2020joint} propose Dual Bandit (DB)~\cite{jeunen2020joint}, a hybrid learning objective that combines both MLE and CRM objective to exploit negative feedbacks in the batch settings. Unlike the batch bandit setting, we focus on the full RL  setting  in this paper, where the user state depends on past actions.  Recently,  batch RL~\cite{levine2020offline} offer a promising direction in the  robotics domain  to leveraging prior experience. Since  most prior off-policy RL algorithms~\cite{mnih2013playing,lillicrap2015continuous,haarnoja2018soft} fail on the batch setting even with even on expert demonstrations, various batch RL algorithms~\cite{fujimoto2019off,kumar2019stabilizing,kumar2020conservative} have been proposed.  We differ from these methods as (1) instead of focus on 
% estimating the true value function as a regression problem, we argue that we need to know the ranking order of the value of candidate items, which is one of the most important characteristics of recommendation. and (2) we propose a new offline ranking algorithm that  can simultaneously maximize the user long-term reward in an unified EM framework.







